PropaInsight: Toward Deeper Understanding of Propaganda in Terms of Techniques, Appeals, and Intent

Propaganda plays a critical role in shaping public opinion and fueling disinformation. While existing research primarily focuses on identifying propaganda techniques, it lacks the ability to capture the broader motives and the impacts of such content. To address these challenges, we introduce propainsight, a conceptual framework grounded in foundational social science research, which systematically dissects propaganda into techniques, arousal appeals, and underlying intent. propainsight offers a more granular understanding of how propaganda operates across different contexts. Additionally, we present propagaze, a novel dataset that combines human-annotated data with high-quality synthetic data generated through a meticulously designed pipeline. Our experiments show that off-the-shelf LLMs struggle with propaganda analysis, but training with propagaze significantly improves performance. Fine-tuned Llama-7B-Chat achieves 203.4% higher text span IoU in technique identification and 66.2% higher BertScore in appeal analysis compared to 1-shot GPT-4-Turbo. Moreover, propagaze complements limited human-annotated data in data-sparse and cross-domain scenarios, showing its potential for comprehensive and generalizable propaganda analysis.

==> content/Downstream.tex <==
\section{Implication: Propaganda Analysis Facilitates Fake News Detection}

\input{figures/fake_news_table}
%\jiateng{Lin and Riya please help to modify this section}

%\heng{Since Longformer-Base works so much better than Flan-T5-Base, maybe we don't need to report Flan-T5-Base results? instead maybe add P and R columns for Longformer-Base}

In this section, we delve deeper into how mastering propaganda analysis can enhance downstream tasks. Specifically, we aim to demonstrate that pre-identifying the components of propaganda frames can enhance our overall assessment of information. We have chosen Fake News Detection~\cite{shu2017fake,zhou2020survey,Fung2021,misinformation2023} as a representative downstream task for this analysis.

To this end, we develop a fake news detection \heng{maybe change 'fake news detection' to 'misinformation detection' throughout the paper} benchmark based on the PoliFact dataset. Each data point in this benchmark is an article labeled as either fake or real. At the same time, these data points also contain propaganda usage, characterized by persuasive techniques within various sentences and appeals designed to captivate readers that aim to advance specific intent. We intend to show that extracting propaganda elements from each article first can further improve the fake news prediction. % made by a base detector.

We employ GPT-4-turbo~\cite{openai2023gpt4} as a baseline for identifying the key elements defined in our propaganda framework. These elements are then used to train traditional Fake News Detectors based on Flan-T5~\cite{chung2024scaling} and Longformer~\cite{beltagy2020longformer}. The models predict the authenticity of propaganda articles using both the original article and the additional propaganda elements identified. As shown in Table~\ref{tab:fake_news_detection}, integrating these key elements into the prediction process resulted in a notable improvement in accuracy.

While any combination of extra propaganda frame elements enhances performance, we specifically observe that including the intent alone can significantly boost the accuracy of fake news detection. We attribute this phenomenon to the crucial nature of intent, as they directly reflect the underlying objectives the author of the propaganda article intends to communicate. We attribute the modest improvement achieved by combining intent with other elements ({\em e.g.,} tactic, appeal) for fake news detection to the limited perception capabilities of the base model detectors. These models likely struggle to simultaneously comprehend the meaning of all elements within a propaganda frame, which can constrain their ability to use this information effectively.









